What is Flagged in Uncertainty Quantification? Latent Density Models for Uncertainty Categorization

Uncertainty Quantification (UQ) is essential for creating trustworthy machine learning models. Recent years have seen a steep rise in UQ methods that can flag suspicious examples, however, it is often unclear what exactly these methods identify. In this work, we propose a framework for categorizing uncertain examples flagged by UQ methods in classification tasks. We introduce the confusion density matrix -- a kernel-based approximation of the misclassification density -- and use this to categorize suspicious examples identified by a given uncertainty method into three classes: out-of-distribution (OOD) examples, boundary (Bnd) examples, and examples in regions of high in-distribution misclassification (IDM). Through extensive experiments, we show that our framework provides a new and distinct perspective for assessing differences between uncertainty quantification methods, thereby forming a valuable assessment benchmark.

==> tex/sec7_legacy.tex <==
\section{Legacy}
\subsection{Other Potential Topics Related}
\paragraph{Input Space Trust Region Detection \textcolor{red}{[for what]}}
We can learn an inverse (pseudo) mapping $g^{-1}$ between hidden space and the input space, such that $g\circ g^{-1}\circ g(x) = g(x),\forall x\in\mathcal{X}$, i.e., the inverse (pseudo) mapping $g^{-1}$ may not learn the identical input as $x$, but instead learns to recover a potentially representative failure mode in the input space. 

However, the problem with this research direction is what can we do with this inverse model $g^{-1}$, since we can on the other hand define trust regions in the latent space much more easily, and predict whether a new sample will be located in a trusted region or not.


\paragraph{Where to Patch Your Model \textcolor{red}{[Ensemble Lit. Rev.]}}
This idea is related to model ensemble: we can train a separated model for those data that are located outside the trusted region.

\paragraph{Latent Space Guided Active Sensing \textcolor{red}{[significance?]}}
Interpretable active sensing policy learning. With the Integrated Jacobian method for the inverse mapping $g^{-1}$, we will be able to interpret the sensing decisions made by doctors: if there are three possible clinical states (e.g., the Alzheimer), and a doctor has scheduled a test, he may want to distinguish between some possible certain hidden states in his mind (i.e., the latent space).

An example: A patient comes with feature $x_1 = 0, x_2 = *, x_3 = *$. Lets assume when $x_1 = 0$, the patient either in clinical state $S_2$ if $x_2 >0$, or in clinical state $S_3$ if $x_3 > 0$.

Here, $S_0$ is the current latent variable with partially observed information, and we want to interpret the decision made by a doctor as what is considered to be the potential latent state when scheduling the measurement.

\subsection{Potential Approaches:}
\begin{itemize}
    \item Epistemic Misclassification: we may need to use hidden representations learned by different layers in defining the extrapolation region.
    \item Aletoric Misclassification: need some experiments to show how are the misclassified examples in the training dataset distributed in the hidden space. Maybe start with MNIST
    \item A simplex generation algorithm: (but think it may have a name in literature): Given a latent space value of a new sample, we may want to generate a simplex that includes this sample, either with the trusted or un-trusted training latent variables (e.g., misclassified examples are marked in the latent space as un-trusted latent variables). For k-dim latent space, we need to find those $k+1$ (un-)trusted variables with a 'growing bubble' method. We can use example-based interpretations for predicted failure cases.
\end{itemize}

\paragraph{Aleatoric misclassification} There is no clear notion of aleatoric misclassification. However, we could argue that an input example $x \in \X$ is likely to be misclassified due to a model ambiguity if the model relates it to other misclassified examples (characterization à la SimplEx). In this case, assume that the model classification does not match the true label: $f(x) \neq y$. We could look for examples in the training set that have been misclassified in a similar way: $\Dmis(x,y) = \{ (x^i,y^i) \in \Dtrain \mid f(x^i) = f(x) \wedge y^i = y\}$. We could then measure how the new example is related to these similarly misclassified example with $p_{\Dmis(x,y)}(x)$, where $p_{\Dmis(x,y)}$ is a density estimated based on $\Dmis(x,y)$ (possibly estimated on top of a model's latent space, like SimplEx). A high value for this density hints that $x$ is in a region where this type of misclassification happens frequently. 


\subsection{A Motivating Example}
We start illustrating the key insight of this work with a motivating example. Figure~\ref{fig:t-sne} shows the t-SNE clustering of latent space variables of a CNN model trained on the MNIST dataset. In the training time, we remove the $0$-class, thus the model is only able to learn to identify digit $1$-$9$. In testing time, we use the vanilla test-time samples
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.45\linewidth]{figs/training.png}
    \includegraphics[width=0.45\linewidth]{figs/testing.png}
    \caption{t-SNE visualization of latent variables learned by CNN model on the MNIST dataset. Left: training w/o class '0', right: testing with class '0'.}
    \label{fig:t-sne}
\end{figure}

\subsection{Training Time Aleatoric Failures}
During training time, it is often the case that we have imperfect model and/or imperfect data, which is potentially due to
\begin{enumerate}
    \item imperfect learning algorithms
    \item overfitting or underfitting
    \item adversarial examples or erroneous labels
\end{enumerate}

Due to either limited capacity of models or imperfectness of labels, a model may only \textit{perform well} in a subset of the training set, which we refer to as \textbf{well-learned} examples. 

Intuitively, a straightforward way in distinguishing between well-learned and not well-learned examples is to check whether their corresponding predictions match training labels, yet such a naive approach can not reason about why and how the model learns to identify this specific subset of examples.

Alternatively in this work, we follow the basic idea of SimplEx~\citep{crabbe2021explaining} by having a deeper look on the latent variables for better model interpretability. 

\begin{reassumption}[restate=,name=Latent Space Continuity]\upshape
\textcolor{red}{We need some mild assumptions like SimplEx, e.g., continuity of the latent space and the linear mapping between latent space and output space in classifiers}
\end{reassumption}

\begin{redefinition}[restate=,name=Latent Local Consistency]\upshape
We define the local consistency of the latent space according to the label distributions in a local area of the latent space, either through 

\textbf{1. Latent Convext Hull}
\textcolor{red}{Computational much more expensive, and seems to be hardly solvable in my very naive approximated try}

With this method, only when an example is enclosed by a convex hull that composed by examples from the same class can it be classified as a non-aleatoric example.

or
\textbf{2. Latent Nearest Neighbors}
\textcolor{red}{much simpler, conducting exps with, currently}

With this method, we search for the $k$-Nearest-Neighbors in the latent space of each training sample to see if they are from the same class. This approach is much simpler to implement and more flexible (we may use different $k$'s to adjust the sensitivity in defining aleatoric examples, while in the former approach it is fixed given the latent space dimension)
\end{redefinition}

\begin{redefinition}[restate=,name=Aleatoric Failures]\upshape
We define the aleatoric failures (and correspondingly, aleatoric examples) in the latent space based on their local consistency.

\end{redefinition}

During tarining time, we can categorize the data into four classes, namely:
\begin{enumerate}
    \item (53436/54077; $98.81\%$, w.r.t. $10$-NN) Consistent Correct Class: e.g., all latent nearest samples of a certain sample '7' are '7', and it is classified to the correct class '7'. $\rightarrow$ idea cases.
    \item (18/54077; $0.03\%$, w.r.t. $10$-NN) Consistent Failure Class: e.g., latent nearest samples of a given sample '7' are all '7', but the sample is misclassified. $\rightarrow$ the last linear layer is problematic.
    \item (480/54077; $0.89\%$,w.r.t. $10$-NN) Inconsistent Correct Class: e.g., latent nearest samples of a given sample '7' have different labels, and the model correctly identifies this sample to be '7' $\rightarrow$ potential aleatoric examples.
    \item (143/54077; $0.26\%$,w.r.t. $10$-NN) Inconsistent Failure Class: e.g., latent nearest samples of a given sample '7' have different labels, but the model failed in identifying this sample to be '7' $\rightarrow$ troublesome aleatoric examples.
\end{enumerate}

\subsection{Testing Time Aleatoric and Epistemic Missclassification}

\begin{redefinition}[restate=,name=Epistemic Failures]\upshape
We define the epistemic examples, in the testing time, based on the continuity assumption we have.
\textcolor{red}{Need to be further formalized}
\end{redefinition}


\begin{table}[!htbp]
\centering
\begin{tabular}{|c|c|c|}
%\hline
%\multicolumn{3}{|c|}{info}\\ % 
\hline
 Consistency & Avg. Dist. to Train. Samp. & Class \\
\hline
 Yes & Large & Epistemic Untrusted \\
\hline
 Yes & Small & Trusted \\
\hline
 No & Large &  Epistemic+Aleatoric  \\
\hline
 No & Small & Aleatoric Untrusted \\
\hline
\end{tabular}
\caption{Test Time}
\end{table}




\subsection{algo `lof' (discarded)}
Hyper-parameters: 

1. $\kappa\in\mathbb{N}^*$ for number of nearest neighbors in defining local consistency in the latent space.

2. $q\in(0,1)$ denotes the quantile we use in identifying whether an example is significantly far away from training samples in the latent space. (which serves as a threshold in the density-based approach.)


\begin{enumerate}
    \item For each training sample $(x^n, y^n)\in \mathcal{D}_{\mathrm{train}}$, we can extend the tuple with its corresponding latent space representation $h^n :=  g(x^n)$ to $(x^n, h^n, y^n)$ to facilitate our discussion in the latent space.
    \item For each class of the training set $k \in [K]$, the empirical distribution of samples with their same-class nearest neighbors in the latent space can be calculated. We use $d^k$ to denote the (sorted) averaged distance for class $k$, $d^k = \{d^k_1,..., d^k_{N_k}\}$, where $N_k$ is the number of examples for class $k$ in the training set.
    \item Defining $\psi_f$ according to the local consistency in latent space as well as the distance with regard to the empirical distribution and the quantile hyper-parameter. The distance between a given testing time example and its nearest neighbors in the latent space is considered to be \textbf{low} as long as it is smaller than the $q$-th empirical quantile of $d^k$.

\end{enumerate}

\section{Approach 2: Distance-Based Approach}

\subsection{Latent Space $k$-distance Approach}

\begin{figure}[h]
\centering
\begin{minipage}[htbp]{0.9\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{figs/fig1pg2.pdf}
\end{minipage}%

\caption{Flow chart of the distance-based approach}
\label{fig:method_den}
\end{figure}


We begin with mirroring the concept of k-distance in the input space introduced by ~\citet{breunig2000lof}, to formally define the $k$-distance in the latent space $\mathcal{H}$. With the notion of $\mathcal{H}_\mathrm{train} := \{ g(x) |x\in \mathcal{D}_\mathrm{train}\}$,
\begin{redefinition}[$k$-distance in $\mathcal{H}_\mathrm{train}$] For any positive integer $k$, the $k$-distance in $\mathcal{H}_\mathrm{train}$ of an input $x\in\mathcal{X}$, denoted as $k$-distance($x|\mathcal{H}_\mathrm{train}$), or $d^H_{\mathcal{H}_\mathrm{train}}(x): \mathcal{X}\rightarrow \mathbb{R}$, is defined as the distance $d^H_{\mathcal{H}_\mathrm{train}}(x):=d(g(x),g(x'))$ between the latent space representation $g(x)$ of $x$, and a latent space representation in $\{g(x')| x' \in \mathcal{D}_{\mathrm{train}}\}$ such that:
\begin{enumerate}
    \item for at least $k$ latent representations of the training set $\{g(x'')|x''\in \mathcal{D}_{\mathrm{train}} \}$ it holds that $d(g(x),g(x'')) \le d(g(x),g(x'))$, and
    \item for at most $k-1$ latent representations of the training set $\{g(x'')|x''\in \mathcal{D}_{\mathrm{train}}\} $ it holds that $d(g(x),g(x'')) < d(g(x),g(x'))$.
\end{enumerate}
\end{redefinition}
Moreover, it is also useful to define the $k$-distance in $\mathcal{H}_c$ within a specific class of examples, i.e., $\mathcal{H}_c := \{g(x) |(x,y) \in \mathcal{D}_\mathrm{train} \wedge \mathrm{class}[y] = c \}$:
\begin{redefinition}[$k$-distance in $\mathcal{H}_c$] For any positive integer $k$, the $k$-distance of an input $x\in\mathcal{X}$ in $\mathcal{H}_c$, denoted as $k$-distance($x|\mathcal{H}_c$), or $d^H_{\mathcal{H}_c}(x): \mathcal{X}\rightarrow \mathbb{R}$, is defined as the distance $d^H_{\mathcal{H}_c}(x):=d(g(x),g(x'))$ between the latent space representation $g(x)$ of $x$, and a latent space representation in $\{g(x')| (x',y') \in \mathcal{D}_{\mathrm{train}}\wedge \mathrm{class}[y'] = c\}$ such that:
\begin{enumerate}
    \item for at least $k$ latent representations of the training set $\{g(x'')| (x'',y'') \in \mathcal{D}_{\mathrm{train}}\wedge \mathrm{class}[y''] = c \}$ it holds that $d(g(x),g(x'')) \le d(g(x),g(x'))$, and
    \item for at most $k-1$ latent representations of the training set $\{g(x'')| (x'',y'') \in \mathcal{D}_{\mathrm{train}}\wedge \mathrm{class}[y''] = c \} $ it holds that $d(g(x),g(x'')) < d(g(x),g(x'))$.
\end{enumerate}
\end{redefinition}



\begin{redefinition}[$k$-Nearest Neighbors of $x$]
Given the $d^H(x)$ of $x\in\mathcal{X}$, the $k$-Nearest Neighbors of $x$, $N_{d^H}(x): \mathcal{X}\rightarrow 2^\mathcal{X}$, contains every training example whose distance from $x$ in the latent space is not greater than $d^H(x)$. 
i.e., $N_{d^H}(x) := \{x'\in\mathcal{X}_{\mathrm{train}}| d(g(x),g(x')) \le d^H(x) \}$ 
These samples $x'$ are called the $k$-Nearest Neighbors of $x$.
\end{redefinition}


\begin{redefinition}[LLC: Local \textit{Label} Consistency in Latent Space]
\label{def:LLC}
Given an example $x\in\mathcal{X}$, if the $k$-Nearest Neighbors of $x$, have the same label, i.e., $k_i =k, \forall x_i \in N_{d^H}(x)$. We call this example $x$ is Locally Label-Consistent in latent space. 
\end{redefinition}

\begin{reremark}
If all examples in the training set are Local Label-Consistent in latent space, they can be easily separated with a set of linear models.
\end{reremark}

However, as we have the linear mapping $l$, instead of using the $k$-Nearest Neighbors, in making classification decisions, we need also take the linear layer into consideration, leading to the definition below:
\begin{redefinition}[LPC: Local \textit{Predictive} Consistency in Latent Space ]
\label{def:LPC}
Given an example $x\in\mathcal{X}$, if the model's prediction of the $k$-Nearest Neighbors of $x$, are identical to their corresponding labels, i.e., $k_i =f(x_i), \forall x_i \in N_{d^H}(x)$. We call this example $x$ is Locally Predictive-Consistent in latent space. 
\end{redefinition}

% \begin{reassumption}(Non-Over-Fitted Model)
% We assume the model is appropriately regularized such that the latent representations learned by the model is generalizable (\textcolor{red}{I'm not sure how (and also if there is a need) to present this assumption (--- more formally definition needed)})
% \end{reassumption} 
% \begin{reremark}
% For over-fitted models, we should be more skeptical about the ``warning'' class. (\textcolor{red}{to be verified in experiments})
% \end{reremark}
According to Definition~\ref{def:LLC} and Definition~\ref{def:LPC}, in-distribution testing time examples can be categorized into three classes:

\begin{table}[h]
\caption{Testing time in-distribution examples can be allocated to three classes.}
\centering
\begin{tabular}{|c|c|c|}
%\hline
%\multicolumn{3}{|c|}{info}\\ % 
\hline
 LLC & LPC & Class \\
\hline
 $\cmark$ & $\cmark$ & \textcolor{Green}{Trusted} \\
\hline
 $\xmark$ & $\cmark$ & \textcolor{orange}{Warning} \\
\hline
%  $\xmark$ & $\cmark$\tablefootnote{For inconsistent samples, the distance is considered to be low only when distances to all classes in the inconsistent neighbor set are low.} &  $*$ \\
% \hline
 $\cmark / \xmark$ & $\xmark$ & \textcolor{red}{Untrusted} \\
\hline
\end{tabular}
\end{table}



\section{Approach 2: Distance-Based Approach}

\begin{figure}[h]
\centering
\begin{minipage}[htbp]{0.9\linewidth}
	\centering
	\includegraphics[width=1\linewidth]{figs/fig1pg2.pdf}
\end{minipage}%

\caption{Flow chart of the distance-based approach}
\label{fig:method_den}
\end{figure}

\subsection{Flagging outliers}

There is a limit to model generalization. One should always be skeptical when the model predicts the class of an example $x \in \X$ that significantly differs from the input examples the model was trained on. In an uncertainty quantification perspective, the predictions for these examples are expected to be associated with a large epistemic uncertainty.

Let us now describe a principled  way to flag these examples that are prone to be misclassified due to a large extrapolation. A natural approach is to adapt the outlier detection formalism of~\citet{breunig2000lof} to our set-up. The idea is simple: for each example $x \in \X$, we introduce a measure of the distance between $x$ and the data manifold underlying $\Dtrain$. This distance should be low whenever the example $x$ resembles one or several examples from the training set $\Dtrain$. Conversely, a high value for this distance indicates that the example $x$ differs from training examples. 

In order to couple our notion of distance to the model $f$ of interest, we use the latent space $\H$ encoded in the feature extractor $g$ from Assumption~\ref{assumption:model_architecture}. In this way, the data manifold will be represented by the latent representation of the training set $\Htrain \equiv \{ h^n = g(x^n) | \ n \in [N] \}$. Our notion of distance will be based on the nearest neighbours of $x$ in latent space. For this reason, it is useful to introduce a permutation $\sigma_x : [N] \rightarrow [N]$ that sorts the training examples in ascending order of distance with respect to $g(x) \in \H$: $\norm{g(x) - g(x^{\sigma_x(n_1)})} \leq \norm{g(x) - g(x^{\sigma_x(n_2)})}$ for all $n_1, n_2 \in [N]$ such that $n_1 < n_2$. In this way, $x^{\sigma_x (k)}$ is the K-th nearest neighbour $x$ in latent space.
With this sorting permutation, we are now ready to define our distance. 

\begin{redefinition}[K-distance] Let $K\in \N^*$ be the number of latent neighbours that we consider in our distance.
The \emph{K-distance in $\H$} of an input $x\in\mathcal{X}$ is a map $\kdistance{\cdot}{\Htrain} : \X \rightarrow \R^+$ defined as the distance between $g(x)$ and its K-th nearest neighbour in latent space:
\begin{align*}
    \kdistance{x}{\Htrain} = \norm{g(x) - g(x^{\sigma_x(K)})},
\end{align*}
where $\sigma_x : [N] \rightarrow [N]$ is a permutation that sorts the training examples in ascending order of distance with respect to $g(x) \in \H$.
\end{redefinition}
\begin{reremark}
Note that $\kdistance{\cdot}{\Htrain}$ is not a distance in the strict mathematical sense since it contains only one argument.
\end{reremark}

With this definition, we clearly see that examples with a high $k$-distance are those who are distant from the training examples in the representation space $\H$.
If a test example $x \in \X$ has a $k$-distance above a predetermined threshold $\tau \in \R$ \textcolor{blue}{(H + e.g., $0.99$ quantile of the empirical distribution for $k$-distance of correctly classified training time examples)}, we consider it as an outlier with respect to the training set. 

\subsection{Flagging Inliers}

It is reasonable to assume that the model $f$ can possibly misclassify examples $x \in \X$ that are similar to training examples and thus have a $k$-distance bellow the predetermined threshold $\kdistance{x}{\Htrain} \leq \tau$. This stems from the fact that the model does not necessarily fit the training set perfectly or that some of these training examples are ambiguous. Note that this characterization has no clear equivalent in an uncertainty quantification perspective. A parallel with aleatoric uncertainty is possible if we consider those misclassfied examples as noisy and aleatoric. However, this parallel is limited as those example could also be misclassified due to the model's limited approximation capacity. 

Let us now describe a principled  way to flag these examples that are prone to be misclassified due to a model imperfection. To do this, we will analyze the K-nearest neighbours of $x$ in latent space $\KNN(x) = \left\{ (x^{\sigma_x(n)} , y^{\sigma_x(n)}) \ \mid \ n \in [K] \right\}$. Clearly, if the nearest neighbours of $x$ contain one or several examples that have been misclassified, it is legitimate to be sceptical about the prediction $f(x)$ for this example. In fact, keeping track of the various misclassifications among the neighbours allows us to have an idea on what the misclassification is likely to be.

In order to make this detection of suspicious examples quantitative, we can split the nearest neighbours in different categories according to their true and predicted labels. More precisely, for each couple of classes $(c_1, c_2) \in [C]^2$, we define the corpus $\misKNN{c_1}{c_2}(x) \equiv \set{(x,y) \in \KNN(x) \mid \class[y] = c_1 \wedge \class[f(x)] = c_2}$ of nearest training examples whose true class is $c_1$ and whose predicted class is $c_2$. We will count the number of elements in each of these corpora to break down the the neighbours of $x$ in different categories. If a big portion of these neighbours correspond to misclassified examples, this should trigger our scepticism about the model's prediction $f(x)$. By aggregating the size of each of these corpora, we arrive at the following definition.

\begin{redefinition}[name=Local Confusion Matrix]
Let $f: \X \rightarrow \Y$ be a model trained with a training set $\Dtrain = \set{(x^n, y^n) \mid n \in [N]}$. Let $g: \X \rightarrow \H$ be the feature extractor from Assumption~\ref{assumption:model_architecture}. The \emph{local confusion matrix} $\dmatrix{\cdot}{\Dtrain}: \X \rightarrow (\R^+)^{C \times C}$ is defined as
\begin{align*}
   \dmatrix[c_1 , c_2]{x}{\Dtrain}  = \frac{1}{K} \left| \misKNN{c_1}{c_2}(x) \right| 
\end{align*}
for all $(c_1, c_2) \in [C]^2$.
\end{redefinition}
\begin{reremark}
The name \emph{local confusion matrix} is chosen to make a parallel with confusion matrices. Like confusion matrices, our confusion density indicates the likelihood of each couple $(c_1, c_2)$, where $c_1$ is the true class and $c_2$ is the predicted class. Unlike confusion matrices, our confusion density provides an instance-wise (i.e. for each $x \in \X$) likelihood for each couple.    
\end{reremark}

By staring at the coefficients of the local confusion matrix, we can quantitatively distinguish two situations where the example $x \in \X$ is likely to be misclassified. The first situation is the one previously mentioned: the latent representation $g(x)$ is close to latent representations of training examples that have been misclassified. In our training confusion matrix, this likelihood that $x$ is related to misclassified training examples is reflected by the off-diagonal elements. This motivates the following definition.

\begin{redefinition}[name=Failure Score \textcolor{red}{H: Under-fit Score?}]
Let $\dmatrix{x}{\Dtrain}$ be the \emph{confusion density matrix} for an example $x \in \X$. We define the \emph{failure score} as the sum of each density corresponding to a misclassification in the confusion density matrix
\begin{align*}
   p_{Fail}(x) = \sum_{c_1=1}^{C} \sum_{c_2 \neq c_1}^C \dmatrix[c_1 , c_2]{x}{\Dtrain}.
\end{align*}
We say that an example is Locally Predictive-Consistent (LPC) if no nearest neighbour is misclassified: $p_{Fail}(x) = 0$
\end{redefinition}

A second situation where a misclassification is likely to happen is when $g(x)$ is close to latent representations of training examples that have been correctly assigned a label that differs from the predicted one $\class{f{x}}$. This typically happens when $g(x)$ is located close to a decision boundary in latent space. In our training confusion matrix, this likelihood that $x$ is related to training examples with different labels is reflected by the diagonal elements. This motivates the following definition.  
\begin{redefinition}[name=Non-Conformity Score]
Let $\dmatrix{x}{\Dtrain}$ be the \emph{confusion density matrix} for an example $x \in \X$ with predicted class $c = \class{f(x)}$. We define the \emph{non-conformity score} as the sum of each density of well-classified examples from a different class
\begin{align*}
   p_{NC}(x) = \sum_{\tilde{c} \neq c}^{C}  \dmatrix[\Tilde{c} , \Tilde{c}]{x}{\Dtrain}.
\end{align*}
We say that an example is Locally Label-Consistent if no nearest neighbour is correctly assigned a different label: $p_{NC}(x) = 0$
\end{redefinition}

\textcolor{red}{Two remarks: 1. We need to find better names than "Failure Score" and "Local Predictive Consistency" as those are a bit misleading. 2. I have changed the definition for LLC in a  way that reflects the First Approach  in which LLC and LPC do NOT overlap (so that we don't have to define a warning class). Bellow are the previous definitions for LLC and LPC suggested by Hao. We could discuss what the best version is.}

\if{
\begin{redefinition}[LLC: Local \textit{Label} Consistency in Latent Space]
\label{def:LLC}
Given an example $x\in\mathcal{X}$, if the $k$-Nearest Neighbors of $x$, have the same label, i.e., $k_i =k, \forall x_i \in N_{d^H}(x)$. We call this example $x$ is Locally Label-Consistent in latent space. 
\end{redefinition}

\begin{reremark}
If all examples in the training set are Local Label-Consistent in latent space, they can be easily separated with a set of linear models.
\end{reremark}

However, as we have the linear mapping $l$, instead of using the $k$-Nearest Neighbors, in making classification decisions, we need also take the linear layer into consideration, leading to the definition below:
\begin{redefinition}[LPC: Local \textit{Predictive} Consistency in Latent Space ]
\label{def:LPC}
Given an example $x\in\mathcal{X}$, if the model's prediction of the $k$-Nearest Neighbors of $x$, are identical to their corresponding labels, i.e., $k_i =f(x_i), \forall x_i \in N_{d^H}(x)$. We call this example $x$ is Locally Predictive-Consistent in latent space. 
\end{redefinition}


\begin{table}[h]
\caption{Testing time in-distribution examples can be allocated to three classes.}
\centering
\begin{tabular}{|c|c|c|}
%\hline
%\multicolumn{3}{|c|}{info}\\ % 
\hline
 LLC & LPC & Class \\
\hline
 $\cmark$ & $\cmark$ & \textcolor{Green}{Trusted} \\
\hline
 $\xmark$ & $\cmark$ & \textcolor{orange}{Warning} \\
\hline
%  $\xmark$ & $\cmark$\tablefootnote{For inconsistent samples, the distance is considered to be low only when distances to all classes in the inconsistent neighbor set are low.} &  $*$ \\
% \hline
 $\cmark / \xmark$ & $\xmark$ & \textcolor{red}{Untrusted} \\
\hline
\end{tabular}
\end{table}
}
\fi


\section{Quantitative Metrics}
In this section we elaborate different metrics we use in performance quantification. It is worth noting that our proposed framework is capable of being integrated with a broad class of algorithms to understand uncertainty and misclassification. And at the same time, our framework can work in isolation with the vanilla classifier, i.e., even with a null uncertainty estimator, our framework itself is able to identify suspicious misclassification.

To this end, we use three different groups of metrics to evaluate 1. the precision and recall of trusted predictions, 2. the precision and recall of detecting suspicious out-of-distribution misclassified samples, 3. the precision and recall of detecting in-distribution misclassification examples, and 4. overall precision and recall of misclassification detection.

%We treat the former two as binary classification tasks and use the \textcolor{red}{Precision-Recall Curves}, and introduce the metric of Model Introspection Score for the latter.



\subsection{Model Introspection Scores (MIS)}
To quantitatively evaluate different approaches, it is necessary to define a metric that can be used to assess the ability in identifying misclassification at models' inference time. In this work, we propose Model Introspection Score (MIS), that encourages the discovery of model imperfectness or epistemic example, e.g., o.o.d. examples, in inference time. Specifically, 
\begin{redefinition}[Model Introspection Score]
MIS is defined over a model $f: \mathcal{X}\rightarrow \mathcal{Y}$. And a post-hoc operator plugged in the model, $\psi_f: \mathcal{X} \rightarrow  [C]^+$, that maps the inference time input $x\in \mathcal{D}_{\mathrm{test}}$ to an extended output space $[C]^+ := [C]\cup \{*\} \cup \{\emptyset\}$, where $\{\emptyset\}$ indicates the o.o.d. class in testing time and $\{*\}$ denotes the suspicious wrong predictions so the operator $\psi_f$ tends not to provide a prediction.
Given the test dataset $\mathcal{D}_{\mathrm{test}} = \{(x^m, y^m)| m\in [M]\}$, MIS is composed by the following components:
\begin{enumerate}
    \item Precision on trusted predictions: $$\frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) = \class[y]) \mathbbm{1}(\psi_f(x) \in[C] )]}{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(\psi_f(x) \in[C] )]}$$
    \item Recall on trusted predictions: $$
    \frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) = \class[y])\mathbbm{1}(\psi_f(x) \in[C] )]}{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) = \class[y] )]}
    $$
    \item Precision for O.O.D. detection: $$\frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(\class[y] \not\in [C])\mathbbm{1}(\psi_f(x) = \emptyset)]}{ \mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}}[\mathbbm{1}(\psi_f(x) = \emptyset)]}$$
    \item Recall for O.O.D. detection: $$\frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(\class[y] \not\in [C])\mathbbm{1}(\psi_f(x) = \emptyset)]}{ \mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}}[\mathbbm{1}(\class[y] \not\in [C])]}$$
    \item Precision for I.D. misclassification prediction:
    $$\frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) \neq \class[y])\mathbbm{1}( \class[y]\in [C] ) \mathbbm{1}(\psi_f(x) =* )]}{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(\psi_f(x) = *)]}$$
    \item Recall for I.D. misclassification prediction:
    $$\frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) \neq \class[y])\mathbbm{1}( \class[y]\in [C] ) \mathbbm{1}(\psi_f(x) =* )]}{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) \neq \class[y] )\mathbbm{1}( \class[y]\in [C] )]}$$
    \item Precision in misclassification prediction:
    $$\frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) \neq \class[y]) \mathbbm{1}(\psi_f(x) \not\in[C] )]}{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(\psi_f(x) \not\in[C] )]}$$
    \item Recall for misclassification prediction:
    $$\frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) \neq \class[y]) \mathbbm{1}(\psi_f(x) \not\in[C] )]}{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(f(x) \neq \class[y] )]}$$
    % \item Error rate for trusted predictions:
    % $$\frac{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\mathbbm{1}(\psi_f(x) \ne \class[y])]}{\mathbb{E}_{(x,y)\sim \mathcal{D}_{\mathrm{test}}} [\psi_f(x) \in[C]]}
    % $$
\end{enumerate}
\end{redefinition}

%where $\alpha$ is the coefficient to punish misclassification in the testing time, $\beta$ is the coefficient to punish wrong discoveries for o.o.d. examples. In general Equation (\ref{eqn:mis_score}) can be extended to more general settings where an importance matrix can be included to assign different bonus/punishment to different type of misclassifications. (e.g., in clinical contexts, misdiagnosing an illness to different easily-confused diseases will expose patients to different levels of risks.)

Noted that the MIS is a metric for both the model $f$ and the post-hoc model imperfectness detection operator $\psi_f$.% $\mathcal{F} := \{f_m:\mathcal{X}\rightarrow \mathcal{Y}|m\in [M]\}$.




\begin{table}[h]
\caption{Experiment results\textcolor{red}{will be moved to the section of experiments}}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
 $\psi_f$ & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 \\
\hline
 $f$ (Null) & $0.89$ & $1.0$ & $0.0$ & - & $0.0$ & - & $0.0$ & -  \\
\hline
 Density & $.$ & $ $ & $ $ & $ $ & $ $ & & & \\
\hline
 MC-Drop & $.$ & $ $ & $ $ & $ $ & $ $ & & & \\
\hline
 Ensemble & $.$ & $ $ & $ $ & $ $ & $ $ & & & \\
\hline
SVI & $.$ & $ $ & $ $ & $ $ & $ $ & & & \\
\hline
DUQ & $.$ & $ $ & $ $ & $ $ & $ $ & & & \\
\hline
\end{tabular}
\end{table}

\textcolor{red}{BB: Use of precision and recall is not motivated. If it is arbitrary, it makes more sense to state any binary classfication metric can be used in the framework, with precision/recall an example and metric we use.}

\textcolor{red}{BB: Where do underfitted vs non-conformal examples come in?}

\textcolor{red}{BB: relate back above definitions to density definitions. E.g. }
We define the outlier flagging function $\psi_o(x;\tau):\mathcal{X}\rightarrow \{0,1\}$:
\begin{equation}
        \psi_o(x; \tau) = \mathbbm{1}(\cproba{x}{\Dtrain}<\tau)
\end{equation}
where $\tau$ is the density threshold. Similarly, let the ...[suspicious example definition etc etc]


% \begin{table*}[h]
% 	\centering
% 	\tiny
% 	%\fontsize{8}{11}\selectfont
% 	\caption{Understanding Model Uncertainty}
% 	\begin{tabular}{cccccccc}
% 		\toprule
% 		\toprule
% 		\multicolumn{1}{c}{\multirow{4}{*}{Class}} & \multicolumn{1}{c}{\multirow{4}{*}{Method}} &\multicolumn{6}{c}{Uncertainty} \cr
% 		\cmidrule(lr){3-8}
% 		  & &\multicolumn{2}{c}{$75\%$}&\multicolumn{2}{c}{$50\%$}&\multicolumn{2}{c}{$25\%$} \cr
% 		  \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
% 		  & &Acc&Prop&Acc&Prop&Acc&Prop \cr
% % 		\multirow{1}{c}{Method}&\multirow{1}{c}{Uncertainty}& \multicolumn{3}{c}{Criteria} \cr
% 		%\cmidrule(lr){3-5}
% 		%& & PC & SC & RE  \cr
% 		\cmidrule(lr){1-8}
% 		\multirow{3}{*}{OOD}
% % MCD uncertain Proportion 0.25 [ 0.   ] [ 0.   ]
% % MCD uncertain Acc 0.25 [0.    ] [0.    ]

% % MCD uncertain Proportion 0.5 [ 0.   ] [ 0.   ]
% % MCD uncertain Acc 0.5 [0.    ] [0.   ]

% % MCD uncertain Proportion 0.75 [ 0.   ] [ 0.   ]
% % MCD uncertain Acc 0.75 [0.     ] [0.    ]
% 		& BNN & $ 0. $ & $  0.106 \pm0.022  $ & $ 0.$& $ 0.150 \pm0.039  $ & $  0. $ & $ 0.285  \pm 0.083  $\cr
% 		& MCD & $ 0. $ & $ 0.057\pm0.016$ & $  0. $& $0.084\pm0.024 $ & $  0.  $ & $0.165 \pm 0.048 $\cr
% 		& DE & $  0.  $ & $ 0.125 \pm 0.006 $ & $  0. $ & $ 0.182 \pm0.013  $ & $  0. $ & $0.351   \pm 0.039  $\cr
% 		\cmidrule(lr){1-8}
		
% 		\multirow{3}{*}{Boundary}
% 		& BNN & $ 0.633 \pm  0.026 $ & $  0.070\pm 0.015 $ & $0.625  \pm 0.029 $& $  0.080\pm 0.020   $ & $0.602  \pm 0.042 $ & $ 0.080   \pm0.024  $\cr
% 		& MCD & $0.672 \pm 0.033   $ & $  0.100  \pm 0.011  $ & $0.648\pm 0.039$& $ 0.112 \pm 0.013 $ & $0.627 \pm0.045 $ & $0.115 \pm0.015 $\cr
% 		& DE & $0.678\pm 0.029  $ & $  0.079 \pm 0.013   $ & $ 0.652  \pm 0.029 $& $  0.085  \pm  0.015 $ & $ 0.613 \pm 0.042 $ & $  0.081\pm 0.015 $\cr
% 		\cmidrule(lr){1-8}
		
% 		\multirow{3}{*}{Unfitted}
% 		& BNN & $0.606  \pm 0.022 $ & $  0.163 \pm 0.018 $ & $  0.587 \pm 0.027  $& $  0.145  \pm 0.026  $ & $ 0.578  \pm 0.053  $ & $ 0.090   \pm 0.032 $\cr
% 		& MCD & $ 0.695  \pm0.036$ & $ 0.086  \pm0.016  $ & $ 0.669 \pm 0.037$& $0.089 \pm  0.015 $ & $0.670  \pm 0.039 $ & $0.064\pm 0.010 $\cr
% 		& DE & $ 0.709  \pm 0.036  $ & $  0.078 \pm 0.012  $ & $ 0.687  \pm  0.027  $& $0.070    \pm  0.011  $ & $  0.662  \pm 0.034   $ & $  0.048  \pm 0.010  $\cr
		
% 		\cmidrule(lr){1-8}
		
% 		\multirow{3}{*}{B\&U}
% 		& BNN & $ 0.553 \pm0.027   $ & $ 0.164 \pm 0.015 $ & $  0.557 \pm 0.025  $& $ 0.148  \pm  0.029  $ & $ 0.560   \pm0.040  $ & $ 0.109  \pm 0.036   $\cr
% 		& MCD & $ 0.646\pm  0.014$ & $  0.155 \pm0.011  $ & $0.623\pm 0.016 $& $  0.180 \pm 0.013 $ & $0.604 \pm0.029 $ & $ 0.175\pm 0.019 $\cr
% 		& DE & $0.648   \pm 0.022  $ & $ 0.169  \pm0.013   $ & $ 0.630  \pm 0.016  $& $ 0.191  \pm 0.015  $ & $  0.592 \pm0.020   $ & $ 0.182  \pm   0.019 $\cr
		
% 		\cmidrule(lr){1-8}
		
% 		\multirow{3}{*}{Trusted}
% 		& BNN & $ 0.721 \pm 0.015 $ & $  0.496\pm 0.022 $ & $  0.687 \pm 0.017  $& $0.477\pm 0.044  $ & $ 0.661  \pm  0.014   $ & $ 0.436 \pm 0.059 $\cr
% 		& MCD & $  0.823 \pm 0.014  $ & $ 0.602 \pm 0.018  $ & $ 0.780 \pm0.016$& $ 0.534 \pm 0.016$ & $0.747 \pm 0.015$ & $  0.482 \pm 0.023$ \cr
% 		& DE & $ 0.779  \pm 0.016   $ & $ 0.549 \pm0.009   $ & $  0.739  \pm0.014   $& $ 0.472 \pm 0.010  $ & $ 0.697\pm 0.015   $ & $ 0.339 \pm  0.024 $ \cr
		
% 		\midrule
% % 		\cmidrule(lr){1-14}
% 		\multirow{3}{*}{Overall}
% 		& BNN & $ 0.592 \pm 0.020 $ & $ 1. $ & $  0.545 \pm 0.030 $& $ 1. $ & $  0.450 \pm 0.055 $ & $  1.  $ \cr
% 		& MCD & $ 0.723\pm 0.021$ & $ 1.  $ & $ 0.662 \pm 0.023 $& $ 1. $ & $ 0.580\pm 0.034 $ & $ 1.  $  \cr
% 		& DE & $ 0.646 \pm 0.013 $ & $ 1.  $ & $ 0.572 \pm 0.012  $& $  1.  $ & $ 0.425 \pm0.028 $ & $  1.  $ \cr
% 		\bottomrule
% 		\bottomrule
% 	\end{tabular}\vspace{0cm}
% 	\label{tab:explain_uncertainty}
% \end{table*}
% \begin{table*}[h]
% 	\centering
% 	\tiny
% 	%\fontsize{8}{11}\selectfont
% 	\caption{Understanding Model Certainty}
% 	\begin{tabular}{cccccccc}
% 		\toprule
% 		\toprule
% 		\multicolumn{1}{c}{\multirow{4}{*}{Class}} & \multicolumn{1}{c}{\multirow{4}{*}{Method}} &\multicolumn{6}{c}{Certainty (Trusted)} \cr
% 		\cmidrule(lr){3-8}
% 		  & &\multicolumn{2}{c}{$25\%$}&\multicolumn{2}{c}{$50\%$}&\multicolumn{2}{c}{$75\%$} \cr
% 		  \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8}
% 		  & &Acc&Prop&Acc&Prop&Acc&Prop \cr
% 		\cmidrule(lr){1-8}
% 		\multirow{3}{*}{OOD}
% 		& BNN & $ 0.$ & $ 0.063 \pm  0.065$ & $  0.$& $ 0.041  \pm0.038  $ & $ 0.$ & $ 0.032 \pm 0.027  $ \cr
% 		& MCD & $  0.  $ & $0.212\pm0.049   $ & $  0. $& $ 0.108  \pm 0.025  $ & $  0. $ & $ 0.073 \pm0.016  $ \cr
% 		& DE & $ 0.  $ & $ 0.010   \pm 0.015 $ & $  0.  $& $ 0.009  \pm 0.012  $ & $  0.  $ & $  0.011 \pm 0.012 $ \cr
% 		\cmidrule(lr){1-8}
		
% 		\multirow{3}{*}{Boundary}
% 		& BNN & $ 0.677 \pm0.157  $ & $ 0.009 \pm 0.005 $ & $  0.653  \pm 0.026 $& $ 0.030 \pm 0.012  $ & $ 0.649 \pm 0.031 $ & $  0.047  \pm0.013   $ \cr
% 		& MCD & $ 0.854 \pm0.066   $ & $ 0.016  \pm 0.005  $ & $ 0.765 \pm0.036 $& $  0.045   \pm0.007   $ & $0.712  \pm0.031 $ & $  0.067 \pm 0.009 $ \cr
% 		& DE & $ 0.822  \pm 0.074  $ & $ 0.019 \pm  0.004 $ & $ 0.762  \pm 0.045  $& $ 0.042  \pm 0.007  $ & $ 0.723  \pm 0.034  $ & $0.058   \pm  0.010  $\cr
% 		\cmidrule(lr){1-8}
		
% 		\multirow{3}{*}{Unfitted}
% 		& BNN & $ 0.736  \pm 0.073  $ & $ 0.082 \pm 0.038 $ & $  0.665   \pm 0.038  $& $  0.141   \pm  0.039 $ & $ 0.632\pm 0.029  $ & $ 0.160  \pm 0.025 $ \cr
% 		& MCD & $   0.947  \pm0.028   $ & $ 0.018   \pm 0.006   $ & $0.787  \pm0.031$& $ 0.049 \pm 0.011  $ & $0.723 \pm0.036$ & $ 0.071 \pm 0.014 $  \cr
% 		& DE & $ 0.873  \pm0.058   $ & $  0.047  \pm  0.016  $ & $ 0.788  \pm 0.054  $& $ 0.071  \pm0.017   $ & $ 0.751  \pm0.043   $ & $ 0.078  \pm  0.014  $\cr
		
% 		\cmidrule(lr){1-8}
		
% 		\multirow{3}{*}{B\&U}
% 		& BNN & $  0.466 \pm 0.076  $ & $ 0.088 \pm 0.060  $ & $  0.523  \pm 0.036  $& $ 0.142  \pm 0.041   $ & $ 0.538 \pm 0.030   $ & $  0.157  \pm 0.022   $ \cr
% 		& MCD & $  0.866  \pm 0.053   $ & $ 0.019   \pm 0.005  $ & $0.748\pm 0.046 $& $ 0.062 \pm 0.008    $ & $0.683 \pm  0.018 $ & $0.104\pm0.010 $ \cr
% 		& DE & $ 0.854  \pm 0.068  $ & $ 0.038  \pm 0.007  $ & $ 0.739  \pm 0.056 $& $ 0.081  \pm0.010   $ & $ 0.698  \pm0.033  $ & $ 0.121  \pm 0.012 $\cr
		
% 		\cmidrule(lr){1-8}
		
% 		\multirow{3}{*}{Trusted}
% 		& BNN & $ 0.927  \pm 0.016  $ & $0.757   \pm0.079  $ & $ 0.867 \pm  0.016 $& $ 0.646 \pm 0.056 $ & $  0.821  \pm  0.016  $ & $ 0.603 \pm 0.032 $ \cr
% 		& MCD & $  0.975   \pm 0.007   $ & $  0.735 \pm  0.039  $ & $ 0.930\pm 0.009$& $ 0.736 \pm 0.016 $ & $0.896 \pm0.010 $ & $ 0.686 \pm 0.015$ \cr
% 		& DE & $ 0.953  \pm 0.012 $ & $ 0.887 \pm 0.021 $ & $ 0.900   \pm  0.014 $& $ 0.796 \pm 0.023  $ & $ 0.862  \pm 0.014   $ & $  0.732 \pm  0.020 $ \cr
		
% 		\midrule
% % 		\cmidrule(lr){1-14}
% 		\multirow{3}{*}{Overall}
% 		& BNN & $ 0.809 \pm 0.068 $ & $ 1. $ & $ 0.747 \pm0.040  $& $ 1.$ & $ 0.711 \pm 0.029 $ & $ 1. $\cr
% 		& MCD& $ 0.764 \pm 0.046 $ & $ 1. $ & $0.804\pm 0.018$& $  1. $ & $0.784\pm 0.012$ & $ 1.  $  \cr
% 		& DE & $ 0.934 \pm  0.017 $ & $ 1.  $ & $  0.864 \pm  0.019 $& $ 1. $ & $ 0.816 \pm0.017  $ & $ 1. $ \cr
% 		\bottomrule
% 		\bottomrule
% 	\end{tabular}\vspace{0cm}
% 	\label{tab:explain_certainty}
% \end{table*}


\clearpage
